Autotelic Reinforcement Learning in Multi-Agent Environments

In the intrinsically motivated skills acquisition problem, the agent is set in an environment without any pre-defined goals and needs to acquire an open-ended repertoire of skills. To do so the agent needs to be autotelic (deriving from the Greek auto (self) and telos (end goal)): it needs to generate goals and learn to achieve them following its own intrinsic motivation rather than external supervision. Autotelic agents have so far been considered in isolation. But many applications of open-ended learning entail groups of agents. Multi-agent environments pose an additional challenge for autotelic agents: to discover and master goals that require cooperation agents must pursue them simultaneously, but they have low chances of doing so if they sample them independently. In this work, we propose a new learning paradigm for modeling such settings, the Decentralized Intrinsically Motivated Skills Acquisition Problem (Dec-IMSAP), and employ it to solve cooperative navigation tasks. First, we show that agents setting their goals independently fail to master the full diversity of goals. Then, we show that a sufficient condition for achieving this is to ensure that a group aligns its goals, i.e., the agents pursue the same cooperative goal. Our empirical analysis shows that alignment enables specialization, an efficient strategy for cooperation. Finally, we introduce the Goal-coordination game, a fully-decentralized emergent communication algorithm, where goal alignment emerges from the maximization of individual rewards in multi-goal cooperative environments and show that it is able to reach equal performance to a centralized training baseline that guarantees aligned goals. To our knowledge, this is the first contribution addressing the problem of intrinsically motivated multi-agent goal exploration in a decentralized training paradigm.

==> sections/related_old.tex <==
Cooperative navigation tasks have been studied under goal-conditioned MARL~\citep{yang2018cm3,mordatch2018emergence}. 
These works differ from ours as goals are externally provided during training and evaluation, with each agent
being individually assigned to a target. 
In contrast, we do not externally provide any goals during training and, during evaluation, we provide a group-level goal and expect from agents to self-organize their assignment of sub-goals.


Intrinsic motivation in MARL has been shown to facilitate cooperation in groups of single-goal RL agents~\citep{du2019liir,jaques2019social}.
Here, rewards encouraging social influence~\citep{jaques2019social} and rewards that disentangle an individual's contributions
from group behavior~\citep{du2019liir} can lead to performances on par with algorithms requiring centralized
training~\citep{foerster2017stabilising,rashid2018qmix,lanctot2017unified}.
These work deviate from our setting as they are not goal-conditioned.

Although some contributions have studied the interaction between autotelic agents and social partners, the latter
usually take the role of a teacher.
For example, \citet{nguyen2014socially} studied how an agent can autonomously
decide how to interact with a teacher agent and 
\citet{colas2020language} couple an autotelic agent with a social partner that provides linguistic descriptions of trajectories.
Our work differs from these approaches as we consider a population of agents with no prior knowledge who jointly learn how to achieve a diversity of goals in the absence of a teacher.






\begin{comment}

In goal-conditioned MARL, goals are commonly provided extrinsically in a supervised process and training is centralized. Under these conditions, it has been shown that a compositional communication protocol can emerge for solving collective navigation tasks \cite{mordatch2018emergence}. In another work, a multi-agent curriculum combined with a mechanism for credit assignment was proven useful \cite{yang2018cm3}. These works further differ from ours as they consider a multi-goal setting, i.e. each agent is assigned with a sub-goal while during evaluation we provide a group-level goal and allow agents to self-organize to an assignment to sub-goals.

Intrinsic motivation in MARL has been shown to facilitate cooperation in groups of single-goal RL agents \citep{du2019liir,jaques2019social}. Here, rewards encouraging social influence \citep{jaques2019social} and rewards that disentangle an individual's contributions from group behavior \citep{du2019liir} can lead to behaviors on par with algorithms requiring centralized training \citep{foerster2017stabilising,rashid2018qmix,lanctot2017unified}.   In contrast, our proposed algoithn, the \algname, does not require intrinsic rewards and considers multiple goals.

Although some contributions have studied the interaction between autotelic agents and social partners, the latter usually take the role of a teacher. For example, the SGIM architecture studied how an IMGEP agent can autonomously decide how to interact with a teacher agent \citep{nguyen2014socially,nguyen2012active}. The IMAGINE architecture \cite{colas2020language} couples an language-based IMGEP agent with a social partner that provides linguistic descriptions of trajectories. The agent is then able to re-interpret these descriptions as linguistic goals and to imagine new goals by leveraging the compositionality of language. Our work differs from these approaches as we consider a population of agents with no prior knowledge and skills who jointly learn how to achieve a diversity of goals in the absence of a teacher.
\end{comment}



